Sufficient Representations for Categorical Variables

Many learning algorithms require categorical data to be transformed into real vectors before it can be used as input. Often, categorical variables are encoded as one-hot (or dummy) vectors. However, this mode of representation can be wasteful since it adds many low-signal regressors, especially when the number of unique categories is large. In this paper, we investigate simple alternative solutions for universally consistent estimators that rely on lower-dimensional real-valued representations of categorical variables that are "sufficient" in the sense that no predictive information is lost. We then compare preexisting and proposed methods on simulated and observational datasets.

==> tables/interactions_regression_forest.tex <==
\begin{tabular}{||c c c c c c c c c c||} 
 \hline
 Param & SPCA&	Perm&MEANS&	FISHER&	PCA&	DEV&	DIFF&	HELMERT	&REPEATED \\ [0.5ex] 
 \hline
\textbf{noise ratio} & & & &  & & & & &\\
 \hline
0.1&	-0.01363&	-0.01391&		-0.01340&	-0.01411&	-0.01419&	0.00003	&-0.00324&	-0.00324&	-0.00321\\
0.25&	-0.04331&	-0.04119&		-0.04243&	-0.04138&	-0.04409&	-0.00001&	-0.00953&	-0.00951&	-0.00942\\
0.5&	-0.09327&	-0.08584&	-0.09329&	-0.08611&	-0.09546&	0.00006&	-0.01937&	-0.01926&	-0.01913\\
1&	-0.16340&	-0.14655&	-0.16318&	-0.14702&	-0.16620&	0.00005&	-0.03165&	-0.03173&	-0.03136\\


 \hline
 \textbf{\# levels}& & & &  & & & & &\\
 \hline
100&	-0.03189&	-0.02551&	-0.03056&	-0.02581&	-0.03442&	0.00012&	0.00286	&0.00281&	0.00284\\
500	&-0.12492&	-0.11824&	-0.12559&	-0.11850&	-0.12556&	-0.00005&	-0.03476&	-0.03469&	-0.03440\\


\hline
 \textbf{\# groups}& & & &  & & & & &\\
 \hline
2&	-0.08595&	-0.08453&	-0.08655&	-0.08481&	-0.08591&	-0.00011&	-0.02069&	-0.02064&	-0.02057\\
10&	-0.07086&	-0.05922&	-0.06960&	-0.05950&	-0.07406&	0.00017	&-0.01120&	-0.01124&	-0.01099\\

 \hline
  \textbf{rhos}& & & & & & & & &\\
 \hline
0.25&	-0.08070&	-0.07767&	-0.08057&	-0.07797&	-0.08230&	0.00014&	-0.01715&	-0.01709&	-0.01695\\
0.5&	-0.07611	&-0.06608	&-0.07558&	-0.06634&	-0.07767&	-0.00008&	-0.01475&	-0.01478&	-0.01461\\


 \hline
 \textbf{P[L \textbar A]} & & & & & & & & &\\ %need to fix this alignment!
 \hline
0.6&	-0.07202&	-0.07376&	-0.07164&	-0.07416&	-0.07230&	0.00005&	-0.01626&	-0.01628&	-0.01609\\
0.9&	-0.07828&	-0.07017&	-0.07801&	-0.07038&	-0.08002&	0.00001	&-0.01563&	-0.01561&	-0.01543\\
1&	-0.08491&	-0.07169&	-0.08457&	-0.07192&	-0.08764&	0.00003&	-0.01596&	-0.01592&	-0.01581\\
 \hline
\end{tabular}

==> tables/interactions_regression_forest2.tex <==
\begin{tabular}{||c c c c c c c c c c c c c||} 
 \hline
 Param & Deviation	&	Difference&		Fisher&		Helmert	&	Perm&		Repeated&		MEANS	&	IRPCA	&	IRWEIGHTS	&	PCA MEANS		&SPCA MEANS		&Multi-Perm\\ [0.5ex] 
 \hline
\textbf{noise ratio}& & & &  & & & & & & & &\\
 \hline
0.10&-0.0030&	0.3813&	1.5788&	0.3824&	1.5654&	0.3787&	1.3330&		-0.3093&	1.4505&	1.3819&	1.4472\\
0.25&-0.0044&	0.7676&	3.5214&	0.7659&	3.5074&	0.7622&	4.1501&	2.3668&	4.3279&	4.1974&	4.2445\\
0.50&-0.0007&	1.7976&	7.8237&	1.7891&	7.8086&	1.7764&	7.6697&		5.9500&	7.9830&	7.7790&	8.0972\\
1.0&-0.0108&	3.3072&	14.2712&	3.3197&	14.2343&	3.2807&	18.7940&	15.4321&	19.0194&	18.8529&	14.3916\\



 \hline
 \textbf{\# levels}& & & &  & & & & & & & &\\
 \hline
100&-0.0086&	-0.2995&	2.7303&	-0.2949&	2.7099&	-0.3026&	3.2343&		2.4928&	3.6603&	3.3822&	2.4621\\
500&-0.0021&	3.5989&	11.8630&	3.5983&	11.8401&	3.5733&	15.4121&		11.7524&	15.4603&	15.4131&	11.1318\\






\hline
 \textbf{\# groups}& & & &  & & & & & & & &\\
 \hline
2&-0.0014&	-2.7204&	-10.1880&	-2.7222&	-10.1668&	-2.7086&	-12.4626&		-9.1964&	-12.4788&	-12.4688&	-8.4586\\
10&0.0108&	-0.8503&	-5.1959&	-0.8524&	-5.1737&	-0.8333&	-6.1496&	-5.0800&	-6.6523&	-6.3020&	-5.5861\\



 \hline
  \textbf{rhos}& & & &  & & & & & & & &\\
 \hline
0.25&-0.0171&	1.7306&	8.2454&	1.7324&	8.2222&	1.7137&	7.2331&	7.4032&	7.4266&	7.3114&	7.6926\\
0.50&0.0055&	1.6492&	6.7242&	1.6512&	6.7039&	1.6365&	10.1079&		7.4685&	10.3263&	10.1727&	6.4058\\






 \hline
 \textbf{P[L \textbar A]} & & & &  & & & & & & & &\\ %need to fix this alignment!
 \hline
0.60&-0.0058&	1.6277&	7.1695&	1.6284&	7.1373&	1.6143&	6.0362&		3.8870&	6.2027&	6.1505&	7.2480\\
0.90&-0.0007&	0.9631&	5.5312&	0.9666&	5.5114&	0.9542&	7.0411&		5.3762&	7.2823&	7.0787&	7.1586\\
1.0&-0.0093&	2.3924&	9.3699&	2.3937&	9.3525&	2.3717&	13.8258&	10.9275&	14.0548&	13.8813&	6.7164\\




 \hline
\end{tabular}


==> tables/interactions_xgboost.tex <==
\begin{tabular}{||c c c c c c c c c c||} 
 \hline
 Param & SPCA&	Perm&MEANS&	FISHER&	PCA&	DEV&	DIFF&	HELMERT	&REPEATED \\ [0.5ex] 
 \hline
\textbf{noise ratio} & & & &  & & & & &\\
 \hline
0.1	&-0.01363&	-0.01391&	-0.01340&	-0.01411&	\textbf{-0.01419}&	0.00003&	-0.00324&	-0.00324&	-0.00321\\
0.25&	-0.04331&	-0.04119&	-0.04243&	-0.04138&	-0.04409&	-0.00001&	-0.00953&	-0.00951&	-0.00942\\
0.5&	-0.09327&	-0.08584&	-0.09329&	-0.08611&	-0.09546&	0.00006&	-0.01937&	-0.01926&	-0.01913\\
1&	-0.16340&	-0.14655&	-0.16318&	-0.14702&	-0.16620&	0.00005&	-0.03165&	-0.03173&	-0.03136\\
 \hline
 \textbf{\# levels}& & & &  & & & & &\\
 \hline
 100&	-0.01333&	-0.00041&	-0.01192&	0.00011&	-0.01447&	-0.00011&	0.00040&	0.00041&	-0.00043\\
500&	-0.01122&	0.00164&	-0.01135&	0.00141&	-0.01181&	0.00005&	0.00105&	0.00105&	0.00175\\
\hline
 \textbf{\# groups}& & & &  & & & & &\\
 \hline
 2&	-0.00373&	0.00093&	-0.00303&	0.00101&	-0.00366&	0.00006&	0.00049&	0.00049&	0.00056\\
10&	-0.02082&	0.00030&	-0.02024&	0.00051&	-0.02262&	-0.00012&	0.00096&	0.00096&	0.00076\\
 \hline
  \textbf{rhos}& & & & & & & & &\\
 \hline
 0.25&-0.00796&0.00021&	-0.00669&	0.00028&	-0.00799&	0.00004&	0.00092&	0.00092&	0.00086\\
0.5&-0.01659&0.00103&	-0.01658&	0.00124&	-0.01829&	-0.00010&	0.00053&	0.00053&	0.00046\\
 \hline
 \textbf{P[L \textbar A]} & & & & & & & & &\\ %need to fix this alignment!
 \hline
 0.6&\textbf{-0.00058}&0.00205&0.00128&0.00243&-0.00022&-0.00012&0.00148&0.00148&0.00157\\
0.9&-0.01477&0.00041&-0.01401&0.00019&\textbf{-0.01568}&-0.00002&0.00069&0.00069&0.00107\\
1&-0.02148&-0.00062&-0.02218&-0.00034&\textbf{-0.02352}&0.00005&0.00000&0.00001&-0.00067\\
 \hline
\end{tabular}

==> tables/interactions_xgboost2.tex <==
\begin{tabular}{||c c c c c c c c c c c c c||} 
 \hline
 Param & Deviation	&	Difference&		Fisher&		Helmert	&	Perm&		Repeated&		MEANS		&	IRWEIGHTS	&	PCA MEANS		&SPCA MEANS		&Multi-Perm\\ [0.5ex] 
 \hline
\textbf{noise ratio}& & & &  & & & & & & & &\\
 \hline
0.10 & 0.0009&	-0.0485&	-0.3591&	-0.0486&	-0.3166&	-0.3573&	-0.6627&	-2.3927&	-0.4544&	-0.5128&	-0.3157\\
0.25 & 0.0064&	-0.0837&	-0.0772&	-0.0838&	-0.0851&	-0.1166&	0.2799&		-1.9180&	0.3840&	0.3230&	-0.1198\\
0.50 & 0.0040&	-0.0334&	-0.0825&	-0.0336&	-0.0060&	0.0045&	2.0590&		-0.5175&	2.3238&	2.1538&	0.0408\\
1.0 & -0.0043&	-0.1007&	0.2048&	-0.1008&	0.2355&	0.2217&	3.7204&		-1.4870&	4.1376&	3.9456&	0.1992\\




 \hline
 \textbf{\# levels}& & & &  & & & & & & & &\\
 \hline
100&0.0091&	-0.0371&	0.0258&	-0.0373&	0.0513&	0.0204&	1.6896&		0.4714&	2.0609&	1.8288&	-0.0308\\
500&-0.0059&	-0.1038&	-0.1337&	-0.1038&	-0.0961&	-0.1055&	1.7037&		-3.4359&	1.8930&	1.8515&	-0.0665\\




\hline
 \textbf{\# groups}& & & &  & & & & & & & &\\
 \hline
2&-0.0105&	-0.0934&	-0.0616&	-0.0935&	-0.0410&	-0.0481&	1.0555&		-3.2613&	1.3310&	1.3028&	-0.0996\\
10&0.0107&	-0.0539&	-0.0507&	-0.0540&	-0.0105&	-0.0403&	2.5185&		0.5512&	2.7927&	2.5305&	0.0022\\




 \hline
  \textbf{rhos}& & & &  & & & & & & & &\\
 \hline
0.25&-0.0042&	-0.0952&	0.0422&	-0.0953&	0.0627&	-0.0290&	0.9606&		1.0941&	1.1126&	1.0220&	-0.0440\\
0.50&0.0063&	-0.0504&	-0.1392&	-0.0506&	-0.0980&	-0.0563&	1.8268&		-2.0592&	2.1233&	1.9850&	-0.0533\\




 \hline
 \textbf{P[L \textbar A]} & & & &  & & & & & & & &\\ %need to fix this alignment!
 \hline
0.6&0.0062&	-0.1268&	-0.2327&	-0.1268&	-0.1714&	-0.1577&	0.2372&		-2.3695&	0.3217&	0.2988&	-0.0513\\
0.9&0.0050&	-0.0627&	-0.0187&	-0.0628&	-0.0167&	-0.0473&	1.9059&		-0.7336&	2.0914&	1.9218&	-0.0412\\
1.0&-0.0045&	-0.0440&	0.0223&	-0.0441&	0.0608&	0.0294&	2.5786&		-1.5631&	3.0402&	2.8591&	-0.0535\\



 \hline
\end{tabular}


==> tables/linear_regression_forest.tex <==
\begin{tabular}{||c c c c c c c c c c c c c||} 
 \hline
 Param & Deviation	&	Difference&		Fisher&		Helmert	&	Perm&		Repeated&		MEANS	&	PAX PCA	&	PAX WEIGHT	&	PCA MEANS		&SPCA MEANS		&Multi-Perm\\ [0.5ex] 
 \hline
\textbf{noise ratio} & & & &  & & & & & & & &\\
 \hline
0.1&	-0.00001&	0.00003&	-0.00803&	0.00040&	-0.01574&	0.00067&	-0.00804&	0.00040&	-0.01562&	0.00067&	-0.007987&	0.000400&	-0.019847&	0.000773&	-0.018566&	0.000733&	-0.002203&	0.000889&	-0.020980&	0.000763&	-0.020078&	0.000765&	-0.012895\\
0.25&	0.00001&	0.00005&	-0.01437&	0.00091&	-0.02811&	0.00148&	-0.01439&	0.00091&	-0.02796&	0.00148&	-0.014333&	0.000910&	-0.050031&	0.001802&	-0.044706&	0.001638&	-0.029473&	0.001339&	-0.050456&	0.001746&	-0.049605&	0.001747&	-0.031021\\
0.5&0.00006	&0.00010&	-0.03135&	0.00207	&-0.05801&	0.00334	&-0.03136&	0.00207&	-0.05781&	0.00333&	-0.031073&	0.002064&	-0.092682&	0.003581&	-0.086355&	0.003309&	-0.072098&	0.002730&	-0.093202&	0.003484&	-0.091893&	0.003458&	-0.065979\\
1&0.00020&	0.00013&	-0.05753&	0.00269&	-0.10652&	0.00435&	-0.05756&	0.00269&	-0.10615&	0.00435&	-0.057168&	0.002682&	-0.168212&	0.006078&	-0.157253&	0.005546&	-0.143724&	0.004937&	-0.168193&	0.005893&	-0.167197&	0.005887&	-0.114673\\

 \hline
 \textbf{\# levels}& & & &  & & & & & & & &\\
 \hline
100&0.00001&	0.00003&	0.00127&	0.00009&	-0.00485&	0.00018&	0.00127&	0.00009	&-0.00470&	0.00018&	0.001341&	0.000082&	-0.036662&	0.001662&	-0.034321&	0.001395&	-0.034345&	0.001690&	-0.038887&	0.001709&	-0.037517&	0.001674&	-0.004191\\
500	&0.00014&	0.00009&	-0.06158&	0.00151&	-0.10785&	0.00256&	-0.06162&	0.00151&	-0.10756&	0.00255&	-0.061279&	0.001506&	-0.132256&	0.003614&	-0.122185&	0.003450&	-0.089078&	0.003446&	-0.130712&	0.003524&	-0.130149&	0.003520&	-0.109776\\


\hline
 \textbf{\# groups}& & & &  & & & & & & & &\\
 \hline
2&0.00011&	0.00009	&-0.03814&	0.00181&	-0.06684&	0.00286	&-0.03818&	0.00181&	-0.06655&	0.00286	&-0.038039&	0.001805&	-0.066086&	0.002791&	-0.073709&	0.002968&	-0.042087&	0.002292&	-0.067424&	0.002838&	-0.067170&	0.002815&	-0.060183\\
10&0.00004&	0.00005	&-0.02257&	0.00125&	-0.04611&	0.00226&	-0.02257&	0.00125&	-0.04594&	0.00225&	-0.022312&	0.001241&	-0.093277&	0.003421&	-0.074081&	0.002887&	-0.075816&	0.003006&	-0.092998&	0.003272&	-0.091243&	0.003288&	-0.054338\\


 \hline
  \textbf{rhos}& & & & & & & & & & & &\\
 \hline
0.25&0.00016&	0.00008&	-0.02893&	0.00169&	-0.05363&	0.00271&	-0.02899&	0.00169&	-0.05341&	0.00270&	-0.028789&	0.001684&	-0.074521&	0.006717&	-0.078977&	0.006756&	-0.073713&	0.006274&	-0.074805&	0.006467&	-0.074245&	0.006514&	-0.059014\\
0.5&-0.00001&	0.00006&	-0.03041&	0.00139	&-0.05741&	0.00243&	-0.03038&	0.00139&	-0.05719&	0.00242&	-0.030180&	0.001387&	-0.080413&	0.002371&	-0.073215&	0.002166&	-0.057029&	0.002029&	-0.080973&	0.002329&	-0.079907&	0.002321&	-0.055425\\


 \hline
 \textbf{P[L \textbar A]} & & & & & & & & & & & &\\ %need to fix this alignment!
 \hline
0.6&0.00010&	0.00008&	-0.03195&	0.00210&	-0.06171&	0.00373	&-0.03199&	0.00211&	-0.06147&	0.00373&	-0.031859&	0.002097&	-0.063272&	0.003635&	-0.064483&	0.003562&	-0.042821&	0.003066&	-0.063784&	0.003586&	-0.063432&	0.003589&	-0.053615\\
0.9&0.00004&	0.00006&	-0.01661&	0.00135&	-0.03409&	0.00223&	-0.01667&	0.00135&	-0.03382&	0.00223&	-0.016537&	0.001344&	-0.079906&	0.004034&	-0.072234&	0.003671&	-0.059294&	0.003452&	-0.079858&	0.003894&	-0.078684&	0.003890&	-0.052344\\
1&0.00009&	0.00009	&-0.04066&	0.00201	&-0.07197&	0.00325&	-0.04062&	0.00201&	-0.07180&	0.00324	&-0.040301&	0.002002&	-0.095396&	0.003825&	-0.084451&	0.003476&	-0.074318&	0.003407&	-0.096454&	0.003766&	-0.094966&	0.003756&	-0.065061\\
 \hline
\end{tabular}

==> tables/linear_regression_forest2.tex <==
\begin{tabular}{||c c c c c c c c c c c c c||} 
 \hline
 Param & Deviation	&	Difference&		Fisher&		Helmert	&	Perm&		Repeated&		MEANS		&	IRWEIGHTS	&	PCA MEANS		&SPCA MEANS		&Multi-Perm\\ [0.5ex] 
 \hline
\textbf{noise ratio} & & & &  & & & & & & & &\\
 \hline
0.10&0.0015&	0.8002&	1.5616&	0.8010&	1.5502&	0.7955&	1.9651&	0.2200&	2.0761&	1.9878&	1.2813\\
0.25&-0.0007&	1.4269&	2.7722&	1.4286&	2.7577&	1.4231&	4.8800&	2.9043&	4.9204&	4.8395&	3.0545\\
0.50&-0.0056&	3.0861&	5.6361&	3.0870&	5.6168&	3.0595&	8.8517&	6.9560&	8.8991&	8.7797&	6.3850\\
1.0&-0.0203&	5.5909&	10.1047&	5.5936&	10.0712&	5.5565&	15.4825&		13.3874&	15.4809&	15.3967&	10.8343\\




 \hline
 \textbf{\# levels}& & & &  & & & & & & & &\\
 \hline
100&-0.0009&	-0.1267&	0.4838&	-0.1274&	0.4686&	-0.1342&	3.5998&		3.3762&	3.8141&	3.6822&	0.4183\\
500&-0.0138&	5.9724&	10.2237&	5.9764&	10.1973&	5.9439&	12.3883&		8.5226&	12.2530&	12.2036&	10.3966\\




\hline
 \textbf{\# groups}& & & &  & & & & & & & &\\
 \hline
2&-0.0112&	3.7419&	6.4653&	3.7458&	6.4383&	3.7325&	6.3949&		4.1214&	6.5201&	6.4964&	5.8407\\
10&-0.0039&	2.2322&	4.5060&	2.2319&	4.4902&	2.2065&	8.9059&		7.3013&	8.8804&	8.7204&	5.2888\\




 \hline
  \textbf{rhos}& & & & & & & & & & & &\\
 \hline
0.25&-0.0158&	2.8516&	5.2218&	2.8577&	5.2009&	2.8378&	7.1812&		7.1062&	7.2076&	7.1556&	5.7307\\
0.50&0.0006&	2.9952&	5.5798&	2.9927&	5.5587&	2.9729&	7.7264&		5.5433&	7.7781&	7.6798&	5.3917\\




 \hline
 \textbf{P[L \textbar A]} & & & & & & & & & & & &\\ %need to fix this alignment!
 \hline
0.6&-0.0102&	3.1448&	5.9847&	3.1488&	5.9617&	3.1357&	6.1312&		4.1917&	6.1792&	6.1462&	5.2203\\
0.9&-0.0035&	1.6474&	3.3511&	1.6533&	3.3257&	1.6401&	7.6797&	5.7570&	7.6752&	7.5668&	5.0998\\
1.0&-0.0088&	3.9844&	6.9439&	3.9805&	6.9284&	3.9499&	9.0987&		7.1623&	9.1949&	9.0597&	6.2990\\


 \hline
\end{tabular}


==> tables/linear_xgboost.tex <==
\begin{tabular}{||c c c c c c c c c c||} 
 \hline
 Param & SPCA&	Perm&MEANS&	FISHER&	PCA&	DEV&	DIFF&	HELMERT	&REPEATED \\ [0.5ex] 
 \hline
\textbf{noise ratio} & & & &  & & & & &\\
 \hline
0.1	&0.00292&	0.00366	&	0.00228&	0.00321&	0.00214&	-0.00015&	0.00034&	0.00034&	0.00294\\
0.25&	-0.00816&	0.00212	&	-0.00798&	0.00247&	-0.00822&	0.00001&	0.00076&	0.00076&	0.00197\\
0.5&	-0.02608&	0.00118	&	-0.02499&	0.00128&	-0.02606&	-0.00001&	0.00055&	0.00055&	0.00206\\
1&	-0.05579&	0.00151	&	-0.05859&	0.00127&	-0.05752&	-0.00005&	0.00061&	0.00061&	0.00108\\
 \hline
 \textbf{\# levels}& & & &  & & & & &\\
 \hline
100&	-0.02159&	0.00216	&	-0.02185&	0.00208&	-0.02221&	-0.00007&	0.00015&	0.00015&	0.00189\\
500&	-0.02196&	0.00207&	-0.02278&	0.00203&	-0.02262&	-0.00003&	0.00098&	0.00098&	0.00214\\

\hline
 \textbf{\# groups}& & & &  & & & & &\\
 \hline
2&	-0.01222&	0.00166	&	-0.01166&	0.00160&	-0.01283&	-0.00006&	0.00080&	0.00080&	0.00174\\
10&	-0.03134&	0.00258	&	-0.03297&	0.00251&	-0.03200&	-0.00004&	0.00033&	0.00033&	0.00229\\

 \hline
  \textbf{rhos}& & & & & & & & &\\
 \hline
0.25&	-0.01307&	0.00171	&	-0.01329&	0.00187	&-0.01310&	-0.00002&	0.00065&	0.00065&	0.00135\\
0.5&	-0.03048&	0.00252	&	-0.03135&	0.00225&	-0.03173&	-0.00008&	0.00048&	0.00048&	0.00267\\

 \hline
 \textbf{P[L \textbar A]} & & & & & & & & &\\ %need to fix this alignment!
 \hline
0.6&	-0.00906&	0.00212	&	-0.00862&	0.00185	&-0.00894&	-0.00004&	0.00103&	0.00103&	0.00239\\
0.9&	-0.02242&	0.00145&		-0.02345&	0.00183	&-0.02371&	-0.00003&	0.00032&	0.00032&	0.00133\\
1&	-0.03385&	0.00278&		-0.03488&	0.00248&	-0.03459&	-0.00008&	0.00034&	0.00035&	0.00231\\
 \hline
\end{tabular}

==> tables/linear_xgboost2.tex <==
\begin{tabular}{||c c c c c c c c c c c c c||} 
 \hline
 Param & Deviation	&	Difference&		Fisher&		Helmert	&	Perm&		Repeated&		MEANS	&		IRWEIGHTS	&	PCA MEANS		&SPCA MEANS		&Multi-Perm\\ [0.5ex] 
 \hline
\textbf{noise ratio}& & & &  & & & & & & & &\\
 \hline
0.10&0.0042&	-0.0332&	-0.3472&	-0.0333&	-0.3956&	-0.3597&	-0.1178&		-1.5158&	-0.1039&	-0.0704&	-0.3628\\
0.25&-0.0020&	-0.1035&	-0.2981&	-0.1036&	-0.2465&	-0.2486&	1.2156&		-0.4656&	1.3018&	1.2710&	-0.2337\\
0.50&-0.0046&	-0.0002&	-0.1433&	-0.0003&	-0.1147&	-0.1309&	3.0536&		0.7391&	3.0815&	3.0720&	-0.1526\\
1.0&0.0004&	-0.0328&	-0.1146&	-0.0329&	-0.1119&	-0.1217&	6.5197&		4.3375&	6.5447&	6.3987&	-0.0797\\


 \hline
 \textbf{\# levels}& & & &  & & & & & & & &\\
 \hline
100&-0.0029&	0.0130&	-0.2167&	0.0129&	-0.1814&	-0.1821&	2.5725&		1.9536&	2.7064&	2.6198&	-0.1797\\
500&0.0017&	-0.1019&	-0.2251&	-0.1019&	-0.2366&	-0.2348&	2.6948&		-0.8188&	2.6111&	2.6335&	-0.2346\\



\hline
 \textbf{\# groups}& & & &  & & & & & & & &\\
 \hline
2&0.0010&	-0.0784&	-0.1579&	-0.0784&	-0.1524&	-0.1474&	1.5208&		-0.7811&	1.6993&	1.6985&	-0.1760\\
10&-0.0018&	-0.0212&	-0.2704&	-0.0214&	-0.2550&	-0.2578&	3.7332&		2.2610&	3.6321&	3.5560&	-0.2383\\



 \hline
  \textbf{rhos}& & & &  & & & & & & & &\\
 \hline
0.25&-0.0005&	-0.0425&	-0.1659&	-0.0426&	-0.1531&	-0.1356&	1.5307&		1.3192&	1.5386&	1.5074&	-0.1699\\
0.50&-0.0005&	-0.0496&	-0.2679&	-0.0496&	-0.2583&	-0.2720&	2.8875&		0.6031&	2.9328&	2.8924&	-0.2444\\



 \hline
 \textbf{P[L \textbar A]}& & & &  & & & & & & & &\need to fix this alignment!
 \hline
0.6&0.0020&	-0.0769&	-0.1984&	-0.0769&	-0.2453&	-0.2246&	1.3543&		-0.5436&	1.3416&	1.4081&	-0.1781\\
0.9&-0.0055&	-0.0578&	-0.2326&	-0.0578&	-0.1777&	-0.1978&	2.8596&	1.0038&	2.8892&	2.8312&	-0.2097\\
1.0&0.0022&	-0.0178&	-0.2247&	-0.0180&	-0.2164&	-0.2100&	3.5522&	1.6514&	3.6448&	3.5308&	-0.2337\\


 \hline
\end{tabular}


==> tables/parameters.tex <==
\begin{tabular}{l|l}
 \hline
 Parameter & Values\\
 \hline
Observations ($n$)   & $5000$ \\
Continuous covariates ($p$)  &   $20$ \\
Rhos ($\rho$) & $0.25$\\
Signal to noise ratio & $.5$ \\
Own-group probability ($p_{L}$) & $.9$ \\
Latent groups ($|\mathcal{L}|$) & $2$, $10$ \\
Observable categories  ($|\mathcal{G}|$)  & $100$, $500$ \\
\hline
\end{tabular}


==> tables/real_data_regression_forest.tex <==
\begin{tabular}{ |c|c|c|c| } 
\hline
Method & Pakistan& Ames& King \\
\hline
Means&	\textbf{8.6477}&		\textbf{1.6565}&		\textbf{8.9399}\\
PCA Means&	7.4097&	 1.4460 &		5.5.8697\\
Multi-Perm.&	7.2221&		-0.9272&		5.1317\\
IR-Weights&	7.3084&		-1.0543&		6.5520\\
SPCA Means&	7.4081&		1.4861&		5.8850\\
Deviation&	0.0496&		0.0082&		0.0729\\
Difference&0.8433&		0.1329&		1.0417\\
Fisher&	7.3036&	0.4953&		5.9979\\
Helmert&	7.4323&		0.5440&		5.7737\\
Permutation&	7.2623&		0.5452&	5.6947\\
Repeated&	7.4005&		0.5802&		5.7739\\



\hline
\end{tabular}

==> tables/real_data_xgboost.tex <==
\begin{tabular}{ |c|c|c|c| } 
\hline
Method & Pakistan& Ames& King\\
\hline
Means&	\textbf{2.2009}&\textbf{1.9675	}&\textbf{	2.7473}\\
PCA Means&	-1.4385&	1.2001&	-0.8828	\\
Multi-Perm.&	0.2826&		-0.5384&		0.8126\\
IR-Weights&	0.6143&		-0.8474&		1.6069\\
SPCA Means&	-1.4584&	1.2705&		-0.8432\\
Deviation&	-0.0542&		0.0873&	0.0114\\
Difference&	0.5288&		0.2160&		0.4088\\
Fisher&	0.0378&		0.3422&		-0.2879\\
Helmert	&-0.2981&		0.3975&	-0.7384\\
Permutation&	0.5285&	0.4260&		-0.8074\\
Repeated&	-0.2981&	0.4020&		-0.7384\\



\hline
\end{tabular}
